FIZZ: Factual Inconsistency Detection by Zoom-in Summary and Zoom-out Document

Through the advent of pre-trained language models, there have been notable advancements in abstractive summarization systems. Simultaneously, a considerable number of novel methods for evaluating factual consistency in abstractive summarization systems has been developed. But these evaluation approaches incorporate substantial limitations, especially on refinement and interpretability. In this work, we propose highly effective and interpretable factual inconsistency detection method metric Factual Inconsistency Detection by Zoom-in Summary and Zoom-out Document for abstractive summarization systems that is based on fine-grained atomic facts decomposition. Moreover, we align atomic facts decomposed from the summary with the source document through adaptive granularity expansion. These atomic facts represent a more fine-grained unit of information, facilitating detailed understanding and interpretability of the summary's factual inconsistency. Experimental results demonstrate that our proposed factual consistency checking system significantly outperforms existing systems.

==> TABLES/analysis_case.tex <==
\begin{table}[hb!]
%\footnotesize % 텍스트 크기를 줄임
\scriptsize
\centering
\small
\setlength{\tabcolsep}{3pt} % 셀 간격을 조정
\renewcommand{\arraystretch}{1.5} % 행 높이를 조정
\begin{tabular}{p{7.5cm}} % 각 열의 폭을 충분히 넓게 설정
\toprule
\textbf{Coreference Resolved Document} \\ \hline
Ancelotti admits facing Simeone is both an 'honour' and a 'problem'.\\ \hline
\textbf{Coreference Resolved Summary} \\ \hline
% \hline
Carlo Ancelotti, italian boss admits facing atletico is both an `honour' and a `problem'\\ 
\hline
\textbf{Atomic Facts (Entailment score)} \\ \hline
Carlo Ancelotti admits facing \textbf{Atletico} is an honour. (0.08)\\ \hline
\textbf{Atomic Facts Candidates (Entailment score)} \\ \hline
% \hline
Carlo Ancelotti admits facing \textbf{simeone} is an honour. (0.60)\\ 
Carlo Ancelotti admits facing \textbf{Vicente Calderon} is an honour. (0.24)\\
\bottomrule
\end{tabular}
\caption{Case of Coreference Resolution}
\vspace{-6mm}
\label{table:case}
%\vspace{15pt} %표 밑 공간 줄이기
\end{table}

==> TABLES/appx_summac_cr.tex <==
\begin{table}[]
    \centering
    \resizebox{\linewidth}{!}{
        \begin{tabular}{l|cc|c}
            \toprule
             & \begin{tabular}[c]{@{}c@{}}\textbf{\textsc{AggreFact-}}\\\textbf{\textsc{Cnn-FtSota}}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{\textsc{AggreFact-}}\\\textbf{\textsc{XSum-FtSota}}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{\textsc{Avg}}\end{tabular} \\
            \midrule
            SummaC-ZS & 64.0$\pm$3.8 & 56.4$\pm$1.2 & 60.2 \\
            SummaC-ZS with CR & 64.7$\pm$2.5 & 56.9$\pm$1.9 & 60.8 \\
            SummaC-ZS with CR \& AF & 70.2$\pm$2.9 & 59.8$\pm$1.8 & 65.0 \\
            \bottomrule
        \end{tabular}
    }
    \caption{Performance of SummaC-ZS with coreference resolution and atomic facts decomposition on \textsc{AggreFact-FtSota} split.}
\label{tab:appx_summac_cr}
% \vspace{-5mm}
\end{table}
